LipCoder: Voice-Enabled Coding Toolkit

AI-assisted programming environments have accelerated software development, giving rise to new paradigms like vibe coding. However, their benefits remain largely inaccessible to visually impaired programmers, as existing screen readers and assistive tools offer limited support for these emerging workflows. We introduce LipCoder, a voice-centric programming toolkit designed to deliver editor-level functionality through auditory and speech-based interfaces. LipCoder offers features comprising speech feedback and earcon cues for comprehension and validation, as well as natural language input for navigation and modification. In an exploratory evaluation, 5 visually impaired programmers performed a series of coding tasks comparing LipCoder with a baseline of VSCode, Copilot, and VoiceOver. Quantitative trends and qualitative feedback point to directions for auditory-first design that may broaden accessibility in speech-driven coding environments.

==> figures/feature_plot.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/quadrant_with_features.png}
    \caption{Enter Caption}
    \label{fig:placeholder}
\end{figure*}

==> main-tagged.tex <==
% Accessible (tagged) build of the MAIN PAPER ONLY (no appendix).
% Compile THIS file instead of main.tex to produce the tagged submission PDF:
%   pdflatex main-tagged  ->  bibtex main-tagged  ->  pdflatex x2
% \DocumentMetadata must appear before \documentclass, hence this wrapper.
%
% Everything else follows from \buildmode; see the BUILD MODE block in main.tex.
% References into the omitted appendix are resolved from appendix-labels.tex,
% a snapshot of the full build's labels -- regenerate it whenever the appendix
% changes (see the note at the top of that file).
\DocumentMetadata{
  lang        = en-US,
  pdfversion  = 1.7,
  testphase   = {phase-III, table, math, firstaid},
}
\def\buildmode{main}
\input{main.tex}


==> sections/8-conclusion.tex <==
\section{Conclusion}
% \\lipcoder contributes a novel step towards inclusive programming by reimagining the coding workflow as an auditory-first, voice-driven experience. We introduced a voice-enabled toolkit that consolidates editing, navigation, and AI assistance into a seamless environment tailored for visually impaired developers – yet we found it can equally benefit sighted programmers by reducing visual context-switching. Through our user study, we showed that blind developers using \lipcoder achieved improved efficiency and felt less cognitive stress compared to a baseline state of practice (combining a screen reader with AI code completion). Furthermore, our findings revealed that \emph{vibe coding} - generation of voice-based conversational, context-sensitive code - is not only viable but can improve productivity and understanding for all users when implemented thoughtfully. In sum, this work bridges the accessibility gap in modern coding tools, showing how speech and sound can serve as first-class interaction mediums in programming.

% Looking ahead, our vision is to foster an ecosystem of accessible and inclusive programming that empowers developers of all abilities through multimodal interfaces. \lipcoder's design principles and empirical insights lay the groundwork for future research to build upon. We encourage the community to expand this paradigm, exploring richer auditory cues, more robust speech interactions, and integration with the full development lifecycle. By continuing to innovate at the intersection of AI, voice technology, and software development, we can move toward a future where everyone, regardless of visual ability, can participate in cutting-edge programming workflows. %We invite further research and development in this space to realize the full potential of voice-enabled coding, ensuring that
% We envision a future where the next generation of IDEs and coding assistants will not only be more intelligent, but also universally accessible.

\lipcoder explores how a unified, voice-enabled programming environment can expand accessibility for visually impaired developers. Our exploratory study suggests that auditory parity and speech-driven coding are feasible and perceived as valuable by visually impaired programmers. Although broader evaluations and long-term deployments are needed, the observed trends and qualitative feedback highlight the potential of auditory-first toolkits in making modern, AI-assisted development more inclusive. We envision a future where the next generation of IDEs and coding assistants will not only be more intelligent, but also universally accessible. By open-sourcing \lipcoder, we aim to foster continued research and collaboration toward accessible, speech-centered programming.

==> tables/dev_env_comparison.tex <==
% \begin{table*}
%   \caption{Comparison of Non-Visual Development Environments. SH: Syntax-aware highlighting, OS: Outline and structure views, L: linting, AR: autocompletion and refactoring, D: Debugging, AI: AI-driven coding assistance}
%   \label{table:dev_env_comparison}
%   \begin{tabular}{lccccccll}
%     \toprule
%     Environment & SH & OS & L & AR & D & AI & Main feature & Integration Level\\
%     \midrule
%     \texttt{StructJumper \cite{}} & 100 & & & & & & Code-structure navigation, AST exploration & Emacs extension \\
%     \texttt{CodeTalk \cite{}} & 100 & \ding{51} & & & & & Token reading \& summarization, indentation/structure navigation & Visual Studio extension \\
%     \texttt{TCS \cite{}}& 300 & & & & &  & Tactile rendering of indentation profiles & Dedicated hardware device\\
%     \texttt{Emacspeak \cite{}}& 400& & & & &  & Menu \& buffer event narration & Built into Emacs\\
%     \texttt{JavaSpeak \cite{}}& 400& & & & &  & Java project navigation & Built into Java IDE\\
%     \texttt{Sodbeans \cite{}}& 400& & & & & & GUI menu navigation, button/event announcements & NetBeans fork\\
%     \texttt{WAD \cite{wad_stefik07}}& 400& & & & & & Control-flow sonification; variable-change timeline & Standalone debugger\\
%     \midrule
%     \texttt{LipCoder \cite{}}& 400& & & & & & Integrates all features above + AI aided semantic reading and writing & Portable VS Code extension\\
%     \bottomrule
%   \end{tabular}
% \end{table*}

\begin{table*}
  \centering
  %\small           
  \setlength{\tabcolsep}{3pt}        % reduce column padding
  \renewcommand{\arraystretch}{1.1}
  \caption{Comparison of Non-Visual Development Environments. 
  SR: Screenreader, PR: Project Overview Readouts, NS: Navigation \& Search, CO: Code Operations, AS: Alerts \& Suggestions, D: Debugging \& Runtime Inspection \textcolor{red}{I have some concerns regarding this table --- are these checkmarks finalized? Or are they just placeholders? It seems like there are too many Xs in here --- this makes the prior works look utterly useless, which, I suspect, is not the case. I think the ``Main feature'' should be renamed to Main purposes? As the key features are also enumerated as SR, PR, NS, ...}
  % SH: Syntax-aware highlighting, OS: Outline and structure views, L: linting, AR: autocompletion and refactoring, D: Debugging, AI: AI-driven coding assistance
  }
  \label{table:dev_env_comparison}
  \begin{tabular}{lC{3.3mm}C{3.3mm}C{3.3mm}C{3.3mm}C{3.3mm}C{3.3mm}C{3.3mm}ll}
    \toprule
    \bf Environment &  SR &  PR &  NS &  CO &  AS &  D &  AI & \bf Main feature & \bf Integration Level\\
    \midrule
    {StructJumper \cite{baker15structjumper}}    &  &  & \ding{51} &  &  &  &  & Structure navigation, AST exploration & Emacs extension \\
    {CodeTalk \cite{potluri18codetalk}}          &  &  &  &  &  &  &  & Token reading \& summary, structure navigation & Visual Studio plugin \\
    {Tactile Code Skimmer \cite{falase19tactile}}&  &  &  &  &  &  &  & Rendering of indentation profiles & Dedicated hardware \\
    {Emacspeak \cite{raman96emacspeak}}          &  &  &  &  &  &  &  & Menu \& buffer event narration & Built into Emacs \\
    {JavaSpeak \cite{smith00javaspeak}}          &  &  &  &  &  &  &  & Java project navigation & Built into Java IDE \\
    {Sodbeans \cite{stefik09sodbeans}}           &  &  &  &  &  &  &  & GUI menu navigation, button/event announcements & NetBeans fork \\
    {Wicked Audio Debugger \cite{stefik07wad}}   &  &  &  &  &  &  &  & Control flow sonification; variable change timeline & Standalone debugger \\
    \midrule
    \bf {\lipcoder (ours)}                            & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & Integrated features leveraging ASR \& TTS & VSCode extension \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/full_result.tex <==
\begin{table*}[t]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.15}
  \caption{Outcomes by task condition and cohort (\emph{mean $\pm$ SD}). 
  Rows show B (Copilot) vs. L (LipCoder). 
  SUS $\uparrow$ (0–100), NASA–TLX $\downarrow$ (0–100), Time $\downarrow$ (min),
  Accuracy $\uparrow$ (\%), Keystrokes $\downarrow$.}
  \label{tab:study_outcomes_CL_multirow}
  \begin{tabular}{l l *{5}{c}|*{5}{c}|*{5}{c}}
    \toprule
    \multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Sys.}} &
      \multicolumn{5}{c|}{\textbf{Visually Impaired} (\(n=5\))} &
      \multicolumn{5}{c|}{\textbf{Sighted} (\(n=20\))} &
      \multicolumn{5}{c}{\textbf{Total} (\(n=25\))} \\
    \cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-17}
    & & SUS$\uparrow$ & NASA$\downarrow$ & Time$\downarrow$ & Acc.$\uparrow$ & Keys
      & SUS$\uparrow$ & NASA$\downarrow$ & Time$\downarrow$ & Acc.$\uparrow$ & Keys
      & SUS$\uparrow$ & NASA$\downarrow$ & Time$\downarrow$ & Acc.$\uparrow$ & Keys \\
    \midrule
    \multirow{2}{*}{\textbf{Basic}}
      & $\mathcal{B}$ & 37.0 ± 12.2 & 61.7 ± 25.1 & 13.1 ± 4.2 & 52.0 ± 48.2 & -- & 38.5 ± 27.0 & 49.1 ± 11.5 & -- & -- & -- & 38.1 ± 23.2 & 53.6 ± 17.8 & 13.1 ± 4.2 & 52.0 ± 48.2 & -- \\
      & $\mathcal{L}$ & \textbf{64.5 ± 13.6} & \textbf{33.9 ± 12.3} & \textbf{10.5 ± 3.6} & \textbf{96.0 ± 8.9} & -- & \textbf{49.0 ± 32.7} & \textbf{38.3 ± 18.3} & -- & -- & -- & \textbf{53.5 ± 28.9} & \textbf{36.7 ± 16.1} & \textbf{10.5 ± 3.6} & \textbf{96.0 ± 8.9} & -- \\
    \midrule
    \multirow{2}{*}{\textbf{Boost}}
      & $\mathcal{B}$ & 41.5 ± 17.0 & 42.2 ± 20.2 & 12.9 ± 2.1 & 100.0 ± 0.0 & -- & 42.7 ± 31.4 & 44.8 ± 18.3 & -- & -- & -- & 42.4 ± 27.4 & 43.8 ± 18.3 & 12.9 ± 2.1 & 100.0 ± 0.0 & -- \\
      & $\mathcal{L}$ & \textbf{70.5 ± 14.7} & \textbf{29.4 ± 12.8} & \textbf{10.7 ± 4.3} & 100.0 ± 0.0 & -- & \textbf{48.8 ± 33.6} & \textbf{41.0 ± 18.2} & -- & -- & -- & \textbf{55.1 ± 30.5} & \textbf{36.9 ± 16.9} & \textbf{10.7 ± 4.3} & 100.0 ± 0.0 & -- \\
    \midrule
    \multirow{2}{*}{\textbf{Debug}}
      & $\mathcal{B}$ & 45.0 ± 15.4 & 36.7 ± 21.5 & \textbf{7.1 ± 3.8} & 100.0 ± 0.0 & -- & 52.1 ± 35.5 & \textbf{28.7 ± 13.5} & -- & -- & -- & 50.0 ± 30.6 & 31.5 ± 16.4 & \textbf{7.1 ± 3.8} & 100.0 ± 0.0 & -- \\
      & $\mathcal{L}$ & \textbf{71.5 ± 17.0} & \textbf{26.1 ± 10.1} & 7.6 ± 5.0 & 100.0 ± 0.0 & -- & \textbf{56.9 ± 36.4} & 29.3 ± 14.1 & -- & -- & -- & \textbf{61.2 ± 32.1} & \textbf{28.2 ± 12.5} & 7.6 ± 5.0 & 100.0 ± 0.0 & -- \\
    \midrule
    \multirow{2}{*}{\textbf{Overall}}
      & $\mathcal{B}$ & 41.2 ± 14.3 & 46.9 ± 23.5 & 11.0 ± 4.3 & 84.0 ± 34.8 & -- & 44.4 ± 31.1 & 40.8 ± 16.8 & -- & -- & -- & 43.5 ± 27.1 & 43.0 ± 19.4 & 11.0 ± 4.3 & 84.0 ± 34.8 & -- \\
      & $\mathcal{L}$ & \textbf{68.8 ± 14.4} & \textbf{29.8 ± 11.4} & \textbf{9.6 ± 4.3} & \textbf{98.7 ± 5.2} & -- & \textbf{51.5 ± 33.5} & \textbf{36.2 ± 17.1} & -- & -- & -- & \textbf{56.6 ± 30.1} & \textbf{33.9 ± 15.5} & \textbf{9.6 ± 4.3} & \textbf{98.7 ± 5.2} & -- \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/nasa-tlx.tex <==
\begin{table}[h]
    \centering
    \caption{Task Load Index (NASA-TLX) across conditions}
    \label{tab:lipcoder-results}
    \begin{tabular}{lcc}
        \toprule
        \textbf{Condition} & \textbf{VSCode+Copilot+VoiceOver} & \textbf{LipCoder} \\
        \midrule
        Base       & 58.3 $\pm$ 28.5  & 19.4 $\pm$ 12.4 \\
        Boost      & 26.4 $\pm$ 14.1 & 21.5 $\pm$ 12.2 \\
        Debugging  & 23.6 $\pm$ 7.6 & 33.3 $\pm$ 25.7 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/prior_work_comparison.tex <==
\begin{table*}
  \centering
  \setlength{\tabcolsep}{2pt}        % reduce column padding
  \renewcommand{\arraystretch}{1.1}
  \caption{Comparison of Non-Visual Development Environments (Features from A to Z).}
  \label{table:dev_env_comparison}
  \begin{tabular}{l*{26}{C{3.3mm}}}
    \toprule
    \bf Environment & A & B & C & D & E & F & G & H & I & J & K & L & M & N & O & P & Q & R & S & T & U & V & W & X & Y & Z \\
    \midrule
    {StructJumper \cite{baker15structjumper}}    & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    {CodeTalk \cite{potluri18codetalk}}          & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    {Tactile Code Skimmer \cite{falase19tactile}}& & & & & & & & & & & & & & & & & & & & & & & & & & \\
    {Emacspeak \cite{raman96emacspeak}}          & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    {JavaSpeak \cite{smith00javaspeak}}          & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    {Sodbeans \cite{stefik09sodbeans}}           & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    {Wicked Audio Debugger \cite{stefik07wad}}   & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    \midrule
    \bf {Baseline}                       & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    \bf {\lipcoder (ours)}                       & & & & & & & & & & & & & & & & & & & & & & & & & & \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/sighted_demographics.tex <==
\begin{table*}
    \caption{Demographics of Sighted Programmers. Each participant's screen reader(s), LLM / vibe coding tools, and main programming languages are sorted in preference (left to right).}
    \label{tab:sighted-demographics}
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.1}
  \resizebox{\textwidth}{!}{

    \begin{tabular}{lllllllllllll}
        \toprule
        
        \multirow{2}{*}[-2pt]{\textbf{ID}} 
        & & \multicolumn{2}{c}{\textbf{General Info.}} 
        & & \multicolumn{3}{c}{\textbf{Development Setup}} 
        & & \multicolumn{3}{c}{\textbf{Coding Experience}} 
        \\
        \cmidrule{3-4}
        \cmidrule{6-8}
        \cmidrule{10-12}
        & & Type of VI & Gender & & Preferred IDE & Screen Reader(s) & LLM / Vibe Coding Tools & & Main Languages & Python & Total \\
        \midrule
        \bf A & & Low Vision & Female & & PyCharm & SR & ChatGPT & & Java, Python & 1 yr & 1.5 yrs \\
        \bf B & & Blind      & Male   & & Nano & VO, SR, NVDA & ChatGPT; Windsurf, Gemini-cli & & Python, JavaScript & 5 yrs & 6 yrs \\
        \bf C & & Low Vision & Male   & & VSCode & VO, SR, JAWS & Gemini; Windsurf & & Python, Swift & 20 yrs & 27 yrs \\
        \bf D & & Blind      & Male   & & VSCode & VO, SR, NVDA & ChatGPT, Gemini; Copilot & & JavaScript, Python & 1 yr & 6 yrs \\
        \bf E & & Blind      & Male   & & XCode & VO, SR, JAWS & ChatGPT & & Objective-C, Python & 6 yrs & 10 yrs \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/small_table.tex <==
\begin{table}
    \caption{Frequency of Special Characters}
    \label{tab:freq}
    \begin{tabular}{ccl}
        \toprule
        Non-English or Math&Frequency&Comments\\
        \midrule
        \O & 1 in 1,000& For Swedish names\\
        $\pi$ & 1 in 5& Common in math\\
        \$ & 4 in 5 & Used in business\\
        $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/stats.tex <==
\begin{table*}[t]
  \centering
  %\scriptsize
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.15}
  \caption{Statistical comparison between Copilot (B) and LipCoder (L): Wilcoxon signed-rank per cohort and task with FDR (q) and effect size (Cohen's dz).}
  \label{tab:study_stats}
  \begin{tabular}{l l c c c c}
    \toprule
    \textbf{Task} & \textbf{Cohort} & \textbf{SUS} & \textbf{NASA} & \textbf{Time} & \textbf{Acc.} \\
    \midrule
    \multirow{3}{*}{\textbf{Base}} & Visually Impaired & p=0.042, q=0.173, dz=4.49 & p=0.080, q=0.239, dz=-1.15 & p=0.414, q=0.705, dz=-0.40 & p=0.129, q=0.281, dz=0.82 \\
     & Sighted & p=0.043, q=0.173, dz=0.77 & p=0.043, q=0.173, dz=-0.87 & p=--, q=1.000, dz=-- & p=--, q=1.000, dz=-- \\
     & Total & p=0.003, q=0.097, dz=1.10 & p=0.010, q=0.127, dz=-0.91 & p=0.414, q=0.705, dz=-0.40 & p=0.129, q=0.281, dz=0.82 \\
    \midrule
    \multirow{3}{*}{\textbf{Boost}} & Visually Impaired & p=0.042, q=0.173, dz=5.59 & p=0.080, q=0.239, dz=-1.08 & p=0.276, q=0.510, dz=-0.60 & p=1.000, q=1.000, dz=0.00 \\
     & Sighted & p=0.199, q=0.397, dz=0.51 & p=0.476, q=0.706, dz=-0.24 & p=--, q=1.000, dz=-- & p=--, q=1.000, dz=-- \\
     & Total & p=0.011, q=0.127, dz=0.87 & p=0.102, q=0.281, dz=-0.48 & p=0.276, q=0.510, dz=-0.60 & p=1.000, q=1.000, dz=0.00 \\
    \midrule
    \multirow{3}{*}{\textbf{Debug}} & Visually Impaired & p=0.042, q=0.173, dz=6.33 & p=0.138, q=0.288, dz=-0.78 & p=0.500, q=0.706, dz=0.09 & p=1.000, q=1.000, dz=0.00 \\
     & Sighted & p=0.426, q=0.705, dz=0.36 & p=0.553, q=0.758, dz=0.05 & p=--, q=1.000, dz=-- & p=--, q=1.000, dz=-- \\
     & Total & p=0.024, q=0.173, dz=0.74 & p=0.572, q=0.763, dz=-0.26 & p=0.500, q=0.706, dz=0.09 & p=1.000, q=1.000, dz=0.00 \\
    \midrule
    \multirow{3}{*}{\textbf{Overall}} & Visually Impaired & p=0.042, q=0.173, dz=10.15 & p=0.080, q=0.239, dz=-1.37 & p=0.500, q=0.706, dz=-0.31 & p=0.129, q=0.281, dz=0.82 \\
     & Sighted & p=0.068, q=0.239, dz=0.68 & p=0.123, q=0.281, dz=-0.51 & p=--, q=1.000, dz=-- & p=--, q=1.000, dz=-- \\
     & Total & p=0.004, q=0.097, dz=1.00 & p=0.017, q=0.163, dz=-0.78 & p=0.500, q=0.706, dz=-0.31 & p=0.129, q=0.281, dz=0.82 \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/sus.tex <==
\begin{table}[h]
    \centering
    \caption{System Usability Scale (SUS) across conditions}
    \label{tab:lipcoder-results}
    \begin{tabular}{lcc}
        \toprule
        \textbf{Condition} & \textbf{VSCode+Copilot+VoiceOver} & \textbf{LipCoder} \\
        \midrule
        Base       & 57.5 $\pm$ 7.2  & 88.3 $\pm$ 7.2 \\
        Boost      & 70.8 $\pm$ 14.4 & 93.3 $\pm$ 4.7 \\
        Debugging  & 71.7 $\pm$ 10.4 & 94.2 $\pm$ 2.9 \\
        \bottomrule
    \end{tabular}
\end{table}
